A Brief Survey on Person Recognition at a Distance

Person recognition at a distance entails recognizing the identity of an individual appearing in images or videos collected by long-range imaging systems such as drones or surveillance cameras. Despite recent advances in deep convolutional neural networks (DCNNs), this remains challenging. Images or videos collected by long-range cameras often suffer from atmospheric turbulence, blur, low-resolution, unconstrained poses, and poor illumination. In this paper, we provide a brief survey of recent advances in person recognition at a distance. In particular, we review recent work in multi-spectral face verification, person re-identification, and gait-based analysis techniques. Furthermore, we discuss the merits and drawbacks of existing approaches and identify important, yet under explored challenges for deploying remote person recognition systems in-the-wild.

==> backup.tex <==
Person recognition at a distance entails recognizing the identity of the individual appearing in the images or videos collected by long-range imaging systems such as drones or surveillance cameras.  However, images collected by long-range cameras often suffer from atmospheric turbulence, blur, low-resolution, illumination, pose etc.  In this paper, we provide a brief survey of recent advances in person recognition at a distance.  In particular, remote gait-based and face-based recognition methods in the visible as well as thermal domain will be reviewed.  Furthermore, we will discuss the merits and drawbacks of existing  approaches and identify promising avenues of research in this rapidly evolving field.

Person recognition is the broad task of using any biometric data to identify an individual. Up close this task can be fairly trivial with the use of clear, unique identifiers, such as fingerprints. However, person recognition at a distance is a much more challenging task. This eliminates many types of biometric data, such as fingerprinting and iris scanning, and increases the difficulty of image based data due to multiple factors including low-resolution, illumination and pose variation. 

\chris{There is still a lot to add to this section}

\section{Methods for Person Recognition at a Distance}
In this section we give an overview of current works for recognizing individuals at a distance. The two main methods for this task are Facial Recognition and Gait Analysis. The majority of these works are in the visible spectrum, but recently there has been more work for facial recognition in the thermal domain, which will be overviewed separately. We will provide an overview of the main datasets for training and evaluation, and the main methods for training models. Evaluation will be covered in section \ref{Evaluation}.

\subsection{Visible Facial Recognition}

Facial recognition in the visible spectrum is the most prevalent method for using biometrics to identify individuals at a distance. Current methods use deep convolutional neural networks to create compact representations, or features, of individuals that are easily storable in large quantities. The features provided by these networks are usually generalize well to unseen individuals, and are robust to minor changes to an individuals appearance. For these reasons facial recognition has become popular in many applications such as security, computer authentication (such as in cellular phones), and missing or wanted persons searches. 

\subsubsection{Visible Facial Recognition Datasets}
Due to facial recognition's popularity, and the wide range of imagery depending on the application, there are a large number of visible face recognition datasets. Here we will discuss the datasets that remain popular in training and evaluation today.
\begin{table*}[t]
\begin{tabular}{|c|c|c|c|c|c|c}
    \hline
    Dataset & Subjects & Images & Avg. Images/Subject & Videos & Avg. Videos/Subject \\
    \hline
    LFW & 5,749 & 13,233 & 2 & 0 & - \\
    \hline
    IJB-B & 1,845 & 21,798 & 6 & 7,011 & 4 \\
    \hline
    IJB-C & 3,531 & 31,334 & 6 & 11,779 & 3 \\
    \hline 
    CALFW & 4,025 & & & 0 & - \\
    \hline
    CPLFW & & & & & \\
    \hline
    AgeDB & 568 & 16,488 & & & \\
    \hline
    MegaFace & 690,573 & 1,027,060 &  & & \\
    \hline
    CFP-FP & & & & & \\
    \hline
    CASIA & & & & & \\
    \hline
    MS1MV2 & 10,000 & 10,000,000 & & & \\
    \hline
    Glint360k & 360,000 & 17,000,000 & & & \\
    \hline
\end{tabular}
\end{table*}

\begin{itemize}
\item IJB-B (July 2017) \cite{ijbb} IARPA Janus Benchmark-B. 1,845 subjects, each with at least one video and two still images. Average of 6 still images, plus 30 video frames and 4 videos per subject
\item IJB-C (2018) \cite{ijbc}
\item LFW (2008) \cite{LFWTech} 1,680 have two or more images, 4069 subjects only have a single image
\item CALFW (Aug 2017) \cite{CALFW}
\item CPLFW \cite{CPLFWTech}
\item AgeDB \cite{moschoglou2017agedb} broken into folds, most popular is AgeDB-30. Generally just used as verification set
\item MegaFace (2016) \cite{kemelmacher2016megaface} mainly meant as a test set 
\item CFP-FP \cite{cfp-paper}


\end{itemize}

\subsubsection{Methods for Visible Facial Recognition}

\subsection{Thermal Facial Recognition}

\subsubsection{Thermal Facial Recognition Datasets}
\chris{Copied straight from TBIOM paper for now, working through}
In recent years, many thermal-visible datasets have been released to support face analysis. Specifically, we discuss datasets with over 100 subjects. Figure \ref{fig:datasets} summarizes a set of publicly released and private MWIR or LWIR face datasets, including the MILAB-VTF(B) dataset presented in this paper.

\begin{itemize}
\item The University of Notre Dame \cite{chen03_und} dataset includes 241 unique identities using visible and LWIR cameras with 4 images per subject at low resolution. 

\item The ULFMT \cite{ghiass2018universite} dataset includes unconstrained capture conditions from 238 subjects. The dataset uses non-time synced video recordings by a MWIR and RGB imaging sensor. 

\item The Natural Visible and Infrared Expression Database (NVIE) \cite{wang2010natural} contains sequences by 238 subjects with diverse facial expressions. The LWIR and grayscale visible image streams were simultaneously recorded and manually time-synchronized.

\item There are two different datasets that have been referred to as the University of Houston (UH) dataset. The most recent version \cite{buddharaju2007physiology} was collected in 2007 with MWIR imaging sensors, containing 7,590 MWIR images from 138 subjects. Previously, \cite{kakadiaris2005multimodal} simultaneously acquires visible, thermal, and range data for 3D model generation of 88 subjects. The thermal IR camera used was not specified, though it is expected to be the same as \cite{bourlai2010methodological}.

\item The ARL Multi-Modal Face Database (MMFD) is composed of two separate collections. The MMFD was originally introduced in \cite{hu2016polarimetric} and was extended in \cite{zhang2019synthesis}. Both collections contain simultaneously acquired visible, LWIR, and Polarimetric LWIR data. The total number of subjects (combined from both collections) is 111. All subjects in this dataset were collected at a range of $\le7.5$ meters indoors, under controlled conditions.

\item The MILAB-VTF(A) dataset was collected by the MILAB team at WVU in 2019. It is composed of multi-pose, dual band (MWIR-Visible) face data of 100 subjects, captured indoors at one standoff distance with variable illumination conditions. The dataset is private and cannot be shared as per the IRB, nor can be used without proper approval.

\item The Tufts Face Database \cite{panetta2018comprehensive} is a multi-modal dataset, capturing 100 subjects using LWIR, NIR, 2D, computer sketches, and 3D point clouds.

\item The ARL-VTF dataset is a large scale visible-thermal dataset, with over 500,000 images from 395 subjects using a synchronized acquisition and stereo arrangement. Variability in expressions, pose, and eye wear are systematically recorded. This dataset was collected indoors at a single stand-off distance under controlled conditions.


\item The MILAB-VTF(B) dataset
\end{itemize}

\subsubsection{Methods for Thermal Facial Recognition}

\subsection{Gait Analysis}
\chris{https://arxiv.org/pdf/2203.04179.pdf and https://arxiv.org/pdf/2206.13732.pdf papers that are probably helpful}
\subsubsection{Visible Gait Analysis Datasets}
\subsubsection{Methods for Gait Analysis Recognition}
Another method for at a distance person identification is though the use of gait information. Although gait recognition is generally not as accurate as top facial recognition algorithms \chris{source}, it does have some advantages. Firstly, gait analysis is able to facial obfuscation, such as from individuals wearing masks. Secondly, it does not require an individual be facing the camera to perform inference on person recognition. Finally, gait analysis can perform inference from lower quality images \cite{makihara2020gait}. These advantages allow gait recognition to be useful in cases where facial recognition may not be a viable option, or can provide support to existing systems. In gait analysis there are two main categories of methods, model-based and model-free, based on whether or not the human body's structure is modeled when processing gait features.

\section{Evaluating Person Recognition Models}\label{Evaluation}

\section{Current Challenges and Open Problems}
